INSCIT: Information-Seeking Conversations with Mixed-Initiative Interactions

In an information-seeking conversation, a user may ask questions that are under-specified or unanswerable. An ideal agent would interact by initiating different response types according to the available knowledge sources. However, most current studies either fail to or artificially incorporate such agent-side initiative. This work presents InSCIt, a dataset for Information-Seeking Conversations with mixed-initiative Interactions. It contains 4.7K user-agent turns from 805 human-human conversations where the agent searches over Wikipedia and either directly answers, asks for clarification, or provides relevant information to address user queries. The data supports two subtasks, evidence passage identification and response generation, as well as a human evaluation protocol to assess model performance. We report results of two systems based on state-of-the-art models of conversational knowledge identification and open-domain question answering. Both systems significantly underperform humans, suggesting ample room for improvement in future studies.

==> tables/archived_data_examples.tex <==
\begin{table}
\centering
\normalsize
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{p{10cm}}
\toprule
\dots \textbf{<U>:} Who is the major competitor of PepsiCo? \\ \midrule
\textbf{<A> (clarification):} Would you like to know PepsiCo's major competitor in the beverage market or the snack food market?  \\
\textbf{<A> (direct answer):} PepsiCo has two main competitors in different market sectors. The Coca-Cola Company is its largest competitor in the beverage market, and Kraft Foods is its largest competitor in the snack foods market. \\\midrule\midrule
\dots \textbf{<U>:} Were the directors involved in any controversy? \\\midrule
\textbf{<A> (relevant info):} I couldn't find anything about them themselves in any controversy but their film, V for Vendetta, had a controversial storyline and themes. \\ \textbf{<A> (direct answer):} The Wachowskis' V for Vendetta was considered to have controversial storyline and themes, but have been both criticized and praised by sociopolitical groups. \\
\bottomrule
\end{tabular}
}
\caption{\label{tab:agent_examples} }
\end{table}

\begin{table}
\centering
\normalsize
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{p{10cm}}
\toprule
\dots \textbf{<U>:} Has Shultz ever been a member of any political parties at all? \\ \midrule
\textbf{<A> (relevant info):} I did not find an affiliation but I did find Schultz's political positions are similar to the Democratic Party platform. \\ \textbf{<A> (direct answer):} Yes, at the start of the 2012 United States presidential election Schultz's name was floated as a potential Democratic candidate. \\\midrule\midrule
\dots \textbf{<U>:} What are some of the health consequences of oats? \\\midrule
\textbf{<A> (clarification):} Oat related health concerns include oat allergies, and gluten-related disorders. Which type of health issue would you like to learn more of? \\ \textbf{<A> (direct answer):} Oat toxicity in people with gluten-related disorders depends on the oat cultivar consumed because the immunoreactivities of toxic prolamins are different among oat varieties. Furthermore, oats are frequently cross-contaminated with the other gluten-containing cereals. Pure oat (labelled as ``pure oat'' or ``gluten-free oat'') refers to oats uncontaminated with any of the other gluten-containing cereals. \\
\bottomrule
\end{tabular}
}
\caption{\label{tab:agent_examples_2} }
\end{table}
